Competitive Equilibrium with Chores: Combinatorial Algorithm and Hardness

We study the computational complexity of finding a competitive equilibrium (CE) with chores when agents have linear preferences. CE is one of the most preferred mechanisms for allocating a set of items among agents. CE with equal incomes (CEEI), Fisher, and Arrow-Debreu (exchange) are the fundamental economic models to study allocation problems, where CEEI is a special case of Fisher and Fisher is a special case of exchange. When the items are goods (giving utility), the CE set is convex even in the exchange model, facilitating several combinatorial polynomial-time algorithms (starting with the seminal work of Devanur, Papadimitriou, Saberi and Vazirani) for all of these models. In sharp contrast, when the items are chores (giving disutility), the CE set is known to be non-convex and disconnected even in the CEEI model. Further, no combinatorial algorithms or hardness results are known for these models. In this paper, we give two main results for CE with chores: 1) A combinatorial algorithm to compute a $(1-\varepsilon)$-approximate CEEI in time $\tilde{\mathcal{O}}(n^4m^2 / \varepsilon^2)$, where $n$ is the number of agents and $m$ is the number of chores. 2) PPAD-hardness of finding a $(1-1/\mathit{poly}(n))$-approximate CE in the exchange model under a sufficient condition. To the best of our knowledge, these results show the first separation between the CEEI and exchange models when agents have linear preferences, assuming PPAD $\neq $ P. Finally, we show that our new insight implies a straightforward proof of the existence of an allocation that is both envy-free up to one chore (EF1) and Pareto optimal (PO) in the discrete setting when agents have factored bivalued preferences.

==> Complexcycle.tex <==
\begin{tikzpicture}[scale=0.77,
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=3mm},
]


%Vertices
\node[squarednode]      (v1)      at (4.75,8.5)                       {$\scriptstyle{(1,v_1)}$};
\node[squarednode]      (v2)      at (5.75,0.5)                       {$\scriptstyle{(2,v_2)}$};
\node[squarednode]      (v3)      at (12.75,8.5)                       {$\scriptstyle{(3,v_3)}$};

\node[squarednode]      (w1)      at (9,4)                       {$\scriptstyle{(\tilde{\ell},w_1)}$};
\node[squarednode]      (w2)      at (9,5.5)                       {$\scriptstyle{(\tilde{\ell},w_2)}$};
\node[squarednode]      (w3)      at (9,7)                       {$\scriptstyle{(\tilde{\ell},w_3)}$};





%Partites
\draw[black, very thick] (3.75,4.55+2) rectangle (5.75,8.5+2);
\node at (4.75,6.25) {$V_1$};
\draw[black, very thick] (4.75,0.5-2) rectangle (6.75,4.45-2);
\node at (5.75,-1.85) {$V_2$};
\draw[black, very thick] (11.75,4.55+2) rectangle (13.75,8.5+2);
\node at (12.75,6.25) {$V_3$};

\draw[black, very thick] (8,8) rectangle (10,3);
\node at (9,1.65) {$V_{\tilde{\ell}}$};



%Dots
\filldraw[color=black!60, fill=black!5, very thick](4.75,10) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](4.75,9.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](4.75,7.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](4.75,7) circle (0.02);


\filldraw[color=black!60, fill=black!5, very thick](5.75,2) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](5.75,1.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](5.75,-0.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](5.75,-1) circle (0.02);

\filldraw[color=black!60, fill=black!5, very thick](12.75,10) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.75,9.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.75,7.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.75,7) circle (0.02);

\filldraw[color=black!60, fill=black!5, very thick](9,3.35) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,4.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,6) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,6.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,7.65) circle (0.02);


%Complexcycle
\draw[<-, ultra thick, blue] (w3) -- (v3);
\draw[<-, ultra thick, blue] (v3) -- (w2);
\draw[<-, ultra thick, blue] (w2) -- (v2);
\draw[<-, ultra thick, blue] (v2) -- (w1);
\draw[<-, ultra thick, blue] (w1) -- (v1);
\draw[<-, ultra thick, blue] (v1) -- (w3);
\end{tikzpicture}


==> MBB-network.tex <==
\begin{tikzpicture}
%Styles
[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
roundnode2/.style={circle, draw=red!60, fill=red!5, very thick, minimum size=7mm},
liner/.style={red,->},
lineb/.style={blue,->},
]

%Rectangles
\node[draw, red, fill= blue!15, text width=3cm] at (-6.5,-0.5) {\textcolor{red}{$p'_i = \sum_{j \in [n]}w_{ij}p_j$}};


\node[draw, red!60, fill= blue!20, text width=3cm] at (-6.5,-2.5) {\textcolor{red}{The capacity of the edges $(b_i,g_j)$ is $\infty$.}};

\node[draw, red!60, fill= blue!20, text width=5cm] at (-6.5,-5.5) {\textcolor{red}{If in an Equality Network $N_p$, the max flow $= \sum \limits_{i\in [n]}{}p_i$ , then $p$ is a market clearing price vector}};




%nodes 


   \node (g1) [roundnode2]   {$g_1$};
   \node (g2) [roundnode2] [below=  of g1]  {$g_2$};
   \node (g3) [roundnode2] [below=  of g2]  {$g_3$};
   \node (g4) [roundnode2] [below=  of g3]  {$g_4$};
   
   \node (t) [roundnode2] [right= of g2] {$t$};

    \node (b1) [roundnode] [left=of g1] {$b_1$};
    \node (b2) [roundnode] [left=of g2]  {$b_2$};
    \node (b3) [roundnode] [left=of g3]  {$b_3$};
    \node (b4) [roundnode] [left=of g4]  {$b_4$};

  \node (s) [roundnode] [left= of b2] {$s$}; 
%Lines 
%source and sink edges
    \draw[lineb] (s)--node[above]{$p'_1$}(b1);  \draw[lineb] (g1)--node[above]{$p_1$}(t);
    \draw[lineb] (s)--node[above]{$p'_2$}(b2);  \draw[lineb] (g2)--node[above]{$p_2$}(t);
    \draw[lineb] (s)--node[above]{$p'_3$}(b3);  \draw[lineb] (g3)--node[above]{$p_3$}(t);
    \draw[lineb] (s)--node[below=10pt]{$p'_4$}(b4);  \draw[lineb] (g4)--node[below=10pt]{$p_4$}(t);

%buyer to good edges

    \draw[liner] (b1)--(g2);
    \draw[liner] (b1)--(g3);
    \draw[liner] (b2)--(g3);
    \draw[liner] (b2)--(g4);
    \draw[liner] (b3)--(g2);
    \draw[liner] (b3)--(g3);
    \draw[liner] (b4)--(g1);


\end{tikzpicture}

==> simplecycle.tex <==
\begin{tikzpicture}[scale=0.9,
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
]


%Vertices
\node[squarednode]      (v1)      at (4.75,8.5)                       {$\scriptstyle{(1,v_1)}$};
\node[squarednode]      (v2)      at (5.75,0.5)                       {$\scriptstyle{(2,v_2)}$};
\node[squarednode]      (v3)      at (12.75,8.5)                       {$\scriptstyle{(3,v_3)}$};

\node[squarednode]      (w1)      at (9,4)                       {$\scriptstyle{(\tilde{\ell},w_1)}$};
\node[squarednode]      (w2)      at (9,5.5)                       {$\scriptstyle{(\tilde{\ell},w_2)}$};
\node[squarednode]      (w3)      at (9,7)                       {$\scriptstyle{(\tilde{\ell},w_3)}$};

\node[squarednode]      (l1)      at (1.95,5.25)                       {$\scriptstyle{(\ell_1,y_1)}$};
\node[squarednode]      (l2)      at (12.05,1.25)                       {$\scriptstyle{(\ell_2,y_2)}$};
\node[squarednode]      (l3)      at (9,11.75)                       {$\scriptstyle{(\ell_3,y_3)}$};





%Partites
\draw[black, very thick] (3.75,4.55+2) rectangle (5.75,8.5+2);
\node at (4.75,6.25) {$V_1$};
\draw[black, very thick] (4.75,0.5-2) rectangle (6.75,4.45-2);
\node at (5.75,-1.85) {$V_2$};
\draw[black, very thick] (11.75,4.55+2) rectangle (13.75,8.5+2);
\node at (12.75,6.25) {$V_3$};
\draw[black, very thick] (8,8) rectangle (10,3);
\node at (9,1.65) {$V_{\tilde{\ell}}$};

\draw[black, very thick] (1,7) rectangle (3,3.5);
\node at (1.5,3.25) {$V_{\ell_1}$};
\draw[black, very thick] (11,3) rectangle (13,-0.5);
\node at (12,-0.75) {$V_{\ell_2}$};
\draw[black, very thick] (8,10) rectangle (10,13.5);
\node at (9,9.75) {$V_{\ell_3}$};


%Dots
\filldraw[color=black!60, fill=black!5, very thick](4.75,10) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](4.75,9.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](4.75,7.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](4.75,7) circle (0.02);


\filldraw[color=black!60, fill=black!5, very thick](5.75,2) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](5.75,1.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](5.75,-0.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](5.75,-1) circle (0.02);

\filldraw[color=black!60, fill=black!5, very thick](12.75,10) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.75,9.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.75,7.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.75,7) circle (0.02);

\filldraw[color=black!60, fill=black!5, very thick](9,3.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,4.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,6) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,6.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,7.5) circle (0.02);

\filldraw[color=black!60, fill=black!5, very thick](1.95,6.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](1.95,5.75) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](1.95,4.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](1.95,3.75) circle (0.02);


\filldraw[color=black!60, fill=black!5, very thick](12.05,2.75) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.05,2) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.05,0.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](12.05,-0.25) circle (0.02);

\filldraw[color=black!60, fill=black!5, very thick](9,13.25) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,12.5) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,11) circle (0.02);
\filldraw[color=black!60, fill=black!5, very thick](9,10.25) circle (0.02);


%Complexcycle
\draw[<-, ultra thick, lightgray] (w3) -- (v3);
\draw[<-, ultra thick, lightgray] (v3) -- (w2);
\draw[<-, ultra thick, lightgray] (w2) -- (v2);
\draw[<-, ultra thick, lightgray] (v2) -- (w1);
\draw[<-, ultra thick, lightgray] (w1) -- (v1);
\draw[<-, ultra thick, lightgray] (v1) -- (w3);

%Simple cycle
\draw[->, ultra thick, blue] (v1)--(l1);
\draw[->, ultra thick, blue] (l1)--(v2);
\draw[->, ultra thick, blue] (v2)--(l2);
\draw[->, ultra thick, blue] (l2)--(v3);
\draw[->, ultra thick, blue] (v3)--(l3);
\draw[->, ultra thick, blue] (l3)--(v1);


\end{tikzpicture}

